Crowdsourcing Question-Answer Meaning Representations

We introduce Question-Answer Meaning Representations (QAMRs), which represent the predicate-argument structure of a sentence as a set of question-answer pairs. We also develop a crowdsourcing scheme to show that QAMRs can be labeled with very little training, and gather a dataset with over 5,000 sentences and 100,000 questions. A detailed qualitative analysis demonstrates that the crowd-generated question-answer pairs cover the vast majority of predicate-argument relationships in existing datasets (including PropBank, NomBank, QA-SRL, and AMR) along with many previously under-resourced ones, including implicit arguments and relations. The QAMR data and annotation code is made publicly available to enable future work on how best to model these complex phenomena.

==> background.tex <==
\section{Background: QA - Driven Predicate-Argument Annotation}

While Previous work in predicate-argument annotation have used 
question-answer pairs as an interpretation of their argument role-labels, 
they usually did so in an implicit manner.
PropBank, for example, associates Arg1 of the ``fear-01'' predicate as the answer to the question ``afraid of what?'' \cite{bonial2014propbank}.

A recent exception is the QA-SRL paradigm \cite{he2015qasrl}, which annotated predicate argument structures with explicit argument-role questions from a predefined question grammar.
Specifically, the grammar enforced that each question would contain exactly one verb from the sentence, in addition to prepositions, auxiliaries, and placeholders from a closed list (e.g., ``someone'', ``somewhere''). The answers in QA-SRL consisted of spans of words from the sentence.
For example, given the sentence: ``Barack Obama flew to Moscow'', a valid QA pair can be:
Who \textbf{flew} somewhere? Barack Obama.

Following, \newcite{he2015qasrl} interpreted each QA pair as denoting a predicate and one of its arguments by positing the verb from the question as the predicate, and the answer as its argument. 
Revisiting the previous example, we would get \textbf{flew}(Barack Obama).
Using this simple annotation scheme they were able to 
get good agreement levels with the much more expensive annotation of PropBank.

However, QA-SRL has certain limitations,  due to the restricted form of its questions.
First, its question grammar is limited to verb-centric questions, and can therefore only capture verb-centric propositions.
Furthermore, the template format required non-trivial amount of annotator training, thereby limiting the scalability of this framework.\footnote{\gabi{Luheng, Luke: Is that true? I remember you mentioning this at some point}}

We address these limitations of QA-SRL by significantly reducing the limitations we put on our questions, and by crowd-sourcing all of our anntoations, as elaborated in the following sections.



==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

==> figures/qg_figure.tex <==
\begin{table}[t]
\centering
\scriptsize
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{.3em}
\begin{tabularx}{\columnwidth}{XX}
\toprule
\multicolumn{2}{c}{\textbf{Sentence:} Many substances enter the sea as a result of human activities.}\\
\midrule
Predicted & Gold (Subset) \\
%\cmidrule(lr){1-1}\cmidrule(lr){2-2}
\midrule
What enter the sea as? & What entered the sea? \\
What do many substances enter the sea? & How many substances enter the sea due to humans?\\
What do many substances enter? &\\
What do the substances enter the sea? &\\
What kind of substances? & What are the general number of substances?  \\
What kind of activities?& Who 's activities? / What kind of activities?\\
What enter the sea as a result? & What enters the sea as a result? \\
& Where do substances enter due to the activities? /Where do they enter? \\
& How much of something enters somewhere? \\
\bottomrule
\end{tabularx}
\caption{Example of Generated Questions. The automatic question generator is able to capture some of the NMOD and VCORE relations, but missed certain VMOD relations such as ``when''. \luheng{this is not from the best model though}}
\label{tab:qg_example}
\end{table}



==> figures/question_relation_types.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
Category                & Percent \\ 
Verb arg/mod            & 49   \\ 
Noun arg/mod            & 25    \\ 
Appositive/copula       & 10    \\ 
Number/unit of measure  & 3     \\ 
Coreference             & 3     \\ 
Name deconstruction     & 2     \\ 
Inferred relation       & 6     \\
Other                   & 2 \\
    }\ylabels
    
\begin{figure}[t]
\hspace{-10pt}
\centering
\begin{tikzpicture}    
    \begin{axis}[
    	   width=.9\columnwidth,
	       height=.45\columnwidth,
	       font=\scriptsize,
            ybar,
            bar width=.45cm,
            legend style={at={(0.6,1)},
                anchor=north,legend columns=-1},
            symbolic x coords={Verb arg/mod, Noun arg/mod, Appositive/copula, Number/unit of measure, Coreference, Name deconstruction, Inferred relation, Other},
            xtick=data,
            x tick label style={rotate=45, anchor=north east, inner sep=0mm},
            nodes near coords,
            %nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%},
            nodes near coords align={vertical},
            axis x line*=bottom,
            axis y line*=left,
            %hide y axis,
            ymin=0,ymax=100,
            ylabel={\% of Questions},
        ]
        \addplot table[x=Category,y=Percent]{\ylabels};
        %\legend{Syntactic}
    \end{axis}
\end{tikzpicture}
\caption{Distribution of the most common semantic phenomena covered by \QA pairs randomly sampled from our dataset.}
\label{fig:question-relation-types}
\vspace{-1em}
\end{figure} 

%\begin{table}[t]
%\small
%\newcolumntype{Y}{>{\centering\arraybackslash}X}
%\begin{tabularx} {\columnwidth}{l c *{1}{Y}}
%\toprule
%Category                & Percent \\ \midrule
%Verb arg/mod            & 49\%    \\ 
%Noun arg/mod            & 25\%    \\ 
%Appositive/copula       & 10\%    \\ 
%Number/unit of measure  & 3\%     \\ 
%Coreference             & 3\%     \\ 
%Name deconstruction     & 2\%     \\ 
%Inferred relation       & 6\%     \\
%Other                   & 2\%     \\
%\bottomrule
%\end{tabularx}
%\caption{Distribution of the most common semantic phenomena covered by \QA pairs randomly sampled from our dataset. \todo{(bar chart? pie chart?)}}
%\label{tab:question-relation-types}
%\end{table}

==> figures/relation_denoting_figure.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
    label & freq \\
    Entity & 52 \\
    SR Name & 27 \\
    Novel relation & 16 \\
    Synonym & 10 \\
    Other & 1 \\
    }\ylabels
    
\begin{figure}[t]
\hspace{-10pt}
\centering
\begin{tikzpicture}    
    \begin{axis}[
    	   width=.9\columnwidth,
	       height=.45\columnwidth,
	       font=\scriptsize,
            ybar,
            bar width=.5cm,
            legend style={at={(0.6,1)},
                anchor=north,legend columns=-1},
            symbolic x coords={Entity, SR Name, Novel relation, Synonym, Other},
            xtick=data,
            x tick label style={rotate=45, anchor=north east, inner sep=0mm},
            nodes near coords,
            %nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%},
            nodes near coords align={vertical},
            axis x line*=bottom,
            axis y line*=left,
            %hide y axis,
            ymin=0,ymax=100,
            ylabel={\% of Questions},
        ]
        \addplot table[x=label,y=freq]{\ylabels};
        %\legend{Syntactic}
    \end{axis}
\end{tikzpicture}
\caption{Categorization of the use of external words in questions}
\label{fig:relation-analysis}
\vspace{-1em}
\end{figure}    

%\begin{table}[t]
%\small
%\newcolumntype{Y}{>{\centering\arraybackslash}X}
%\begin{tabularx} {\columnwidth}{l c *{1}{Y}}
%\toprule
%Category                    & Percent \\ \midrule
%Type of an entity           & 52\%    \\ 
%Explicit semantic role name & 27\%    \\ 
%Novel relation              & 16\%    \\ 
%Synonym                     & 10\%    \\ 
%Other                       & ...\%   \\ \bottomrule
%\end{tabularx}
%\caption{Categorization of the use of relation-denoting words in questions (\todo{Percentages are slightly off.. will fix, and change to bar chart})}
%\label{tab:relation-analysis}
%\end{table}


==> figures/words_dist.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
label & freq \\
    what            & \pctWhat{} \\
    who             & \pctWho{} \\
    how             & \pctHow{} \\
    where           & \pctWhere{} \\
    when            & \pctWhen{} \\
    which           & \pctWhich{} \\
    whose           & \pctWhose{} \\
    why             & \pctWhy{} \\
    }\whlabels
    

\begin{figure}[t]
\hspace{-10pt}
\centering
\begin{tikzpicture}    
    \begin{axis}[
    	   width=.9\columnwidth,
	       height=.45\columnwidth,
	       font=\scriptsize,
            ybar,
            bar width=.45cm,
            legend style={at={(0.6,1)},
                anchor=north,legend columns=-1},
            symbolic x coords={what, who, how, where, when, which, whose, why},
            xtick=data,
            %x tick label style={rotate=45, anchor=north east, inner sep=0mm},
            nodes near coords,
            %nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%},
            nodes near coords align={vertical},
            axis x line*=bottom,
            axis y line*=left,
            %hide y axis,
            ymin=0,ymax=100,
            ylabel={\% of Questions},
        ]
        \addplot table[x=label,y=freq]{\whlabels};
        %\legend{Syntactic}
    \end{axis}
\end{tikzpicture}
\caption{Distribution of wh-phrases among questions.}
\label{fig:wh-breakdown}
\vspace{-1em}
\end{figure}    

%\begin{table}[t]
%\small
%\newcolumntype{Y}{>{\centering\arraybackslash}X}
%\begin{tabularx} {\columnwidth}{l c *{4}{Y}}
%\toprule
%Question word   & Percent of data \\ \midrule
%what            & \pctWhat{} \\
%who             & \pctWho{} \\
%how             & \pctHow{} \\
%where           & \pctWhere{} \\
%when            & \pctWhen{} \\
%which           & \pctWhich{} \\
%whose           & \pctWhose{} \\
%why             & \pctWhy{}  \\ \bottomrule
%\end{tabularx}
%\caption{Distribution of wh-phrases among questions. \todo{better visualization: circle chart, bar graph, or sunburst chart}}
%\label{tab:wh-breakdown}
%\end{table}


==> modeling.tex <==
\section{Modeling}
\label{sec:modeling}


%To support future efforts on broad-coverage semantic parsing, we designed two modeling task based on our annotation paradigm: question generation (QG) and question answering (QA).
To establish initial baselines, we apply existing neural models to the QG and QA subtasks as defined in Section~\ref{sec:tasks}. Our baselines solve the two tasks separately and the QA model receives gold questions as input.
%Together, the two task can close the loop of language understanding using the form of natural language QA pairs. Intuitively, given a sentence, an agent that understands the meaning of the sentence should have the power to: 1) propose questions targeting existing semantic relations in the sentence; and 2) answer the questions using words from the sentence, thus completing the relation. %Although recent work has shown good performance
%The form of natural language Q/A pairs also enables easier active learning or human-in-the-loop methods.

\paragraph{Question generation}
%The goal for QG is to generate a set of strings $q_1, \ldots, q_k$ that are answerable given information in the sentence. 
%The major challenge for this task is the large number of different questions that can be asked per sentence. 
Our question generation model learns a mapping from a sentence $\mathbf{w}$ to a set of questions  $q_1,\ldots, q_m$.
%covering the underlying \PA structures (although we are not explicitly modeling them),
We first enumerate pairs of words $(w_{\text{q}}, w_{\text{a}})$ from the sentence as \textit{prompts} to be used in the input, indicating the generated question should target a predicate-argument relationship between these words, if one exists. 
At training time, each training sample is a tuple $(\mathbf{w}, w_{\text{q}}, w_{\text{a}}, q)$, where $q$ is a human-annotated question and $w_{\text{q}}, w_{\text{a}}$ are words from the sentence that occur in the question and answer string, respectively. We then add a set of negative samples, where the output is a single special \textit{NOQ} token indicating that no question can be generated from the prompt.
%If no question is aligned to the prompt, the model generates a special \textit{NOQ} token.

%The output of our model is a set of natural language questions, which is to be evaluated against a set of human-annotated questions. We use automatic evaluation of precision and recall, using on exact string match and fuzzy match (with multi-bleu $> 0.8$).

%\paragraph{Model} 
We use an encoder-decoder model with a copying mechanism \cite{zhou2017neural} to generate questions given an input sentence with part-of-speech tag features and the pair of words tagged.
%with \textit{Q,A} indicating the $w_\text{q}$ and $w_\text{a}$ words, 
At test time, we enumerate all pairs of content words $(w_i, w_j)$ such that $|i - j| \leq 5$ and take the set of generated questions as our prediction, which is then compared against a set of gold questions.
%\luke{how is the binary decision made to not generate a question, when appriorate? or, is the best one always generated and you just have a score cutoff?} \luheng{i looked at the scores, they don't seem to correlate with question quality very well, we might need an explicit reranking model if we want to do this appropriately. ...}

On the QAMR test set, we achieve 31.9\% precision and 19.1\% recall with fuzzy matching (multi-BLEU\footnote{An average of the BLEU1--BLEU4 scores.} $>0.8$), and 8.2\% precision and 4.9\% recall with exact string matching. As discussed in Section~\ref{sec:open-vocab}, the space of QAMR questions contains most of the information of its correponding predicate-argument structure, making the QG problem challenging.

%Table \ref{tab:qg_example} show an example of generated questions from the QAMR development set.

%We evaluate
%Given an input sentence, we first enumerate a pair of words $(w_q, w_a)$ from the sentence, such that the model could learn to generate different questions given each word pair. %Table~\ref{tab:baseline_results} shows the generation results.

%\paragraph{Results}

\paragraph{Question answering}
Although qualitatively different in content and complexity, the format of our question-answering subtask is similar to other reading comprehension tasks, such as SQuAD \cite{rajpurkar2016squad}.\footnote{For the comparison, we filled in non-contiguous answer spans and removed 13 documents from QAMR that overlap with SQuAD.}
Therefore, we can directly apply an existing question-answering model\cite{seo2016bidirectional} to address our QA task, and use the SQuAD evaluation metric. %For a comparison between the tasks, we also run a SQuAD-trained model on the QAMR data and vice versa. %\luheng{Might need to cut this if we don't think it brings new understanding to QAMR} 

%
On the QAMR test set, our model achieved 70.8\%  exact match and 79.7\% F1 score. We can further improve performance to 75.7\% exact match and 83.9\% F1 by pooling our training set with the SQuAD training data.
%Table \ref{tab:baseline_results} shows the performance of our QA models. 
%The model does better in general on QAMR than SQuAD, which is expected: 
%the context in QAMR is a single sentence, so the answer space is much smaller, and the questions are mostly simple and often align closely to their answers.
This suggests that in QAMR, QA is relatively easy compared to QG, since most of the challenge of modeling QAMRs lies in generating the questions.
%What is more striking is that the model trained on SQuAD has reasonable performance on QAMR, while the model trained on QAMR does much worse on SQuAD.
%This bears out the intuition that QAMR---or, \PAS---is in some sense a subtask of reading comprehension.
%\todo{Say something about how it is still a difficult task, but it has a higher ceiling, and it is important.}

%\input{figures/qg_figure}

%\begin{table}[t]
%\centering
%\small
%\newcolumntype{Y}{>{\centering\arraybackslash}X}
%\setlength{\tabcolsep}{.3em}
%\begin{tabularx}{\columnwidth}{l c *{4}{Y}}
%\toprule
%Answering
%    & \multicolumn{2}{c}{\textbf{QAMR-Tes}t}
%    & \multicolumn{2}{c}{\textbf{SQuAD-Dev}}\\
%    \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
%    & \multicolumn{1}{c}{Exact} & \multicolumn{1}{c}{F1}
%    & \multicolumn{1}{c}{Exact} & \multicolumn{1}{c}{F1} \\
%\midrule
%SQuAD-trained   & 50.8 & 65.3   & 67.7  & 77.3 \\
%QAMR-trained    & 70.8 & 79.7   & 40.4  & 50.7 \\
%Combined        & 75.7 & 83.9   & 68.3  & 77.4 \\
%\bottomrule
%\end{tabularx}
%\caption{
%Results for the QA subtask in terms of exact match and F1.
%Question answering results are on the QAMR test set and SQuAD dev set using the SQuAD evaluation metrics of exact match and F1. Results show that our QA subtask is easier than reading comprehension tasks such SQuAD, yet cannot be easily solved using the other dataset.}
%\label{tab:baseline_results}
%\vspace{-1em}
%\end{table}


%\subsection{Question and answer generation}
%\paragraph{Model}
%\paragraph{Results}

==> tasks.tex <==
\section{Formal Task Definitions}
\label{sec:tasks}

\input{figures/structure_figure}

%The\footnote{\gabi{I think that an intro to this section would help its flow, something like: ``In this section we survey the different subtasks involved in sentence-level question answering ...'' and then a high level overview of the subtasks.}} information in our dataset lies in both the choice of the questions to ask and the answers themselves. For example, given the sentence \textit{``John went to the store yesterday.''}, the question \textit{When did John go?} indicates the presence of a temporal modifier on \textit{go} and indicates \textit{John} as the \textit{go}er, and the answer \textit{yesterday} corresponds to the actual semantic argument. 

\paragraph{QAMR Parsing} 
The problem of \textit{QAMR Parsing} is to map a sentence  $\mathbf{w}=w_1, \dots, w_n$ to a set $\mathcal{M}=\{(q_i,a_i) \vert i=1\ldots m\}$ of questions $q_i$ paired with answers $a_i$, such that each $q_i$ contains  a word $w_i$ from the input and each answer $a_i$ is a subsequence of $\mathbf{w}$. Figure~\ref{fig:intro} shows an example $(\mathbf{w},\mathcal{M})$ pair. In Section~\ref{sec:modeling}, we present baselines for the two QAMR parsing subtasks defined below.

{\em Question generation} (QG) involves mapping a sentence $\mathbf{w}$ to a set of questions $\{q_i \vert i=1\ldots m\}$, such that each $q_i$ contains a $w_i \in \mathbf{w}$. The goal is to include every question that is answerable from $\mathbf{w}$, thereby recovering a complete set of predicate-argument relationships. This QG task is closely related to recent work in question generation for reading comprehension~\cite{heilman2010good,mostafazadeh2016generating,du2017learning}, but the QAMR approach differs in its emphasis on coverage.
%\footnote{\julian{Also, the focus on coverage is different?}}
%In Section~\ref{sec:modeling}, we present a neural QG  model for this task, demonstrating that our data support learning question generation models, but the problem is very difficult overall and will require significant future work.

{\em Question answering (QA)} involves mapping a sentence $\mathbf{w}$ and QAMR question $q$ to an output answer $a$, which is a subsequence of $\mathbf{w}$. It is closely related to work in reading comprehension~\cite{seo2016bidirectional,chen2016thorough}, but again targets a different distribution of input questions. 
%In Section~\ref{sec:modeling}, we evaluate performance of existing machine comprehension models to quantitatively measure these differences and point to interesting directions for future work. As we will see, in comparison to QG, QA is a relatively easy task where higher accuracies can be achieved with existing models. It seems to be much easier for current models to find arguments than to determine which semantic relationships are present in $\mathbf{w}$. %\footnote{\luheng{I'm hedging between putting some of the insights here or move them to the modeling section.}}

\paragraph{QAMR Graphs}
We also define the related task of \textit{QAMR graph construction}, to produce structures that more closely resemble previously studied predicate-argument representations. Given a sentence $\mathbf{w}$ and QAMR $\mathcal{M}=\{(q_i,a_i) \vert i=1\ldots m\}$, the goal is to produce a graph $\mathcal{G}$ with subspans of $\mathbf{w}$ as nodes and edges that are labeled with questions $q_i$. Each edge points from a span in $q_i$ to the subgraph of $\mathcal{G}$ that spans the corresponding answer $a_i$. Figure~\ref{fig:struct} shows an example graph for the QAMR in Figure~\ref{fig:intro}. 
Section~\ref{sec:structure} provides a simple heuristic algorithm which builds high quality QAMR graphs.

%along with a qualitative analysis comparing the outputs to several widely studied alternative predicate-argument representations. 

%We show in \autoref{sec:structure} that simple heuristics can be used to build \PAS out of a set of \QA pairs. Two related tasks are developing methods to intelligently build \PAS from \QA pairs and methods to predict these \PA structures directly from a sentence. This task could be accomplished directly by structure prediction methods or by pipelining a \QA generation system with a system that converts a distribution over \QA pairs to the desired structures.


%Formally\footnote{\gabi{Maybe this can be the first paragraph in this section? The current first one seems a bit out of context for me.}}, the question generation task takes as input a sequence of tokens \(w_1, \dots, w_n\) and outputs a \textit{set} of question strings \(\{q_1, \dots, q_m\}\), and a \textit{set} of answer strings \(\{a_1, \dots, a_m\}\), where each question and answer string should have some overlap with the original sentence token \todo{formalize this}. 

%We argue that, a system that understands the meaning of a sentence should be able to propose a set of questions as well as pointing out the corresponding answers. %This is a highly challenging task because it needs to 1) figure out the semantic relations and 2) represent the relations the form of natural language. As an initial step, we breakdown this task into a variety of different subtask, each of which highlighting different modeling challenges.

%The \QA pairs that we gather are rich enough to be useful for a variety of modeling tasks.

%\subsection{Question Generation (QG) }
%Much of the information in our dataset\footnote{\gabi{Maybe it's better to refrain from mentioning the dataset at this point? Since we didn't present it yet, I think it might be better to refer to the task for now}} is in the choice of questions to ask about each sentence.  
%The question generation task is about asking a set of questions given an input sentence, such that the questions are \textit{exhaustive, grammatical}, as well as \textit{answerable}. 
%This makes our QG different from previous reading comprehension dataset \cite{rajpurkar2016squad}, or QASRL \cite{he2015qasrl}, our data covers a large set of different questions for each sentence. 
%
%In many cases, most of the information indicating the \PA arc denoted by a \QA pair is in the question itself, which often categorizes its answers, as in questions beginning with ``When'', ``Where'', ``What size'', ``How many'', etc. This means that for question \luheng{todo}
%
%\note{(This is useful because a lot of SRL information is contained in the questions, because it's the most difficult step towards inducing PAS, and because it can be used for gathering data more cheaply.)}
%Formally, the question generation task takes as input a sequence of tokens
%\(w_1, \dots, w_n\)
%and outputs a \textit{set} of question strings
%\(\{q_1, \dots, q_m\}\).
%As a stand-alone subtask, its performance may be measured by precision and recall based metrics with fuzzy question matching or other measures that compare the output \textit{distribution} of questions with human-annotated data. 

%To draw an analogy with traditional SRL, this task can be understood as: given a sentence, find all the predicates $p_1, \ldots, p_k$ as well as all the possible semantic relations $r_{i,1}, \ldots, r_{i,m_i}$ of each of the predicates $p_i$. In addition, the QG system also has to express each predicate-relation pair $(p_i, r_{i,j})$ in the form of natural language.

%It is also possible to 
%\todo{(Also could employ question answering systems or the crowd in evaluation.)}

%\subsection{Question Answering (QA)}

%Another task associated with our data is question answering. While other tasks with similar formulation \cite{rajpurkar2016squad,richardson2013mctest} focus on reading comprehension and multi-sentence inference, our questions are simpler, directly targeting \PA structure, while at the same time has a broader coverage. %\todo{numbers indicating no. questions per sentence}, 
%and mostly relate to \PA structure instead, as we will show in later sections.

%In the sense of modeling \PA structures, this task is also analogous to the following: given a predicate and a semantic relation, what is the argument?
%\todo{(One way of framing this relationship is saying that a question asks: ``given a predicate and a role, what is the argument?'' But of course, questions contain more information than this, with no clear predicate identification and a fuzzy notion of roles.)}
%\subsection{Generating \QA Pairs}
%The most complete task relating to the dataset is to model the distribution of \QA pairs. This looks much like question generation, and can be done jointly or by pipelining a question generation and question answering model.


